Memory-augmented Dense Predictive Coding for Video Representation Learning

The objective of this paper is self-supervised learning from video, in particular for representations for action recognition. We make the following contributions: (i) We propose a new architecture and learning framework Memory-augmented Dense Predictive Coding (MemDPC) for the task. It is trained with a predictive attention mechanism over the set of compressed memories, such that any future states can always be constructed by a convex combination of the condense representations, allowing to make multiple hypotheses efficiently. (ii) We investigate visual-only self-supervised video representation learning from RGB frames, or from unsupervised optical flow, or both. (iii) We thoroughly evaluate the quality of learnt representation on four different downstream tasks: action recognition, video retrieval, learning with scarce annotations, and unintentional action classification. In all cases, we demonstrate state-of-the-art or comparable performance over other approaches with orders of magnitude fewer training data.

==> sec/background.tex <==
\section{Background}
\noindent In practise, 
the contrastive self-supervised training is formulated as applying a classifier to distinguish between samples drawn from 
joint distribution or from the product of marginals $p(x)p(y)$.\\
\begin{align}
\mathcal{L} = \mathbb{E} \left[ \frac{1}{K} \sum_{i=1}^K log \frac{e^{f(x_i, y_i)}}{\frac{1}{K} \sum_{j=1}^{K} e^{f(x_j, y_j)}}  \right]
\end{align}
where the expectation is over $K$ independent samples $\{ (x_i, y_i) \}_{i=1}^K$ from the joint distribution $p(x,y)$.
In other words, for each $x_i$, one has to predict which of the $K$ samples $y_1, \dots, y_k$ it was jointly drawn with.
This is done using a \emph{critic} function $f(x,y)$ that ideally assigns high values when $(x,y)$ are drawn from the joint, 
and low values when they are drawn from the product of marginals. \\



\begin{comment}
When we begin to consider perception as an information-handling process,
it quickly becomes clear that much of the information received by our brain is highly \emph{redundant},
\ie~portions of the field are highly predictable from other portions.
The preceding statement, 
taken in its broadest implications, is precisely equivalent to an assertion that the world we know is full of regularities.
We may reasonably suppose that a contour, 
the direction of which changes at a constante rate, \ie~the arc of a circle,
could be extrapolated.
Any sort of physical invariance whatsoever constitutes a source of redundancy, \eg~first order, second, or even higher orders.
In other words, 
we can make better-than-chance inferences with respect to the prior and subsequent states received.
One of the goals for self-supervised learning is to abstract these invariances and utilize them properly.\\

\noindent
Percerving the brain as a prediction machine has become the dominant model in cognitive neuroscience in the last decades.
It is conjectured that brains are not always passively awaiting the next waves of sensory stimulation.
Instead, they are pro-active prediction engines constantly trying to anticipate the shape of the incoming sensory signal.
If an agent learns to predict the future, it can take anticipatory actions, 
plan through its predictions, and use prediction as proxy for representation learning.
In cognitive neuroscience, 
this ability has been discovered in the brain, termed as the predictive coding~(also known as predictive processing).
It is a theory of brain function in which the brain is constantly generating and updating a mental model of the environment. 
The model is used to generate predictions of sensory input that are compared to actual sensory input. 
This comparison results in prediction errors that are then used to update and revise the mental model.\\
\end{comment}
